Towards Proper Contrastive Self-supervised Learning Strategies For Music Audio Representation

The common research goal of self-supervised learning is to extract a general representation which an arbitrary downstream task would benefit from. In this work, we investigate music audio representation learned from different contrastive self-supervised learning schemes and empirically evaluate the embedded vectors on various music information retrieval (MIR) tasks where different levels of the music perception are concerned. We analyze the results to discuss the proper direction of contrastive learning strategies for different MIR tasks. We show that these representations convey a comprehensive information about the auditory characteristics of music in general, although each of the self-supervision strategies has its own effectiveness in certain aspect of information.

==> tab_genre.tex <==
\begin{table}[t!]
% \vskip 0.15in
\begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{lcccc}
\textit{Feature} & \textit{dim.} & \textit{SVM} & \textit{LR} \\ 
\hline
\hline
MFCC & 40 & 0.397  & 0.401 \\ 
\hline
% Siamese-{\textit{track-}}_{\textit{Triplet Margin}} & 256 & 0.375 & 0.366 \\ 
% Siamese-{\textit{adjacent-}}_{\textit{Triplet Margin}} & 256 & 0.351 & 0.360   \\ 
% \hline
Siamese-\textit{Self-aug}-\tiny{\textit{InfoNCE}} & 256 & 0.409 & 0.418  \\ 
Siamese-\textit{Self-aug}-\tiny{\textit{InfoNCE-Multi}} & 1280 & 0.373 & 0.413 \\ 
\hline
Siamese-\textit{Adjacent}-\tiny{\textit{InfoNCE}} & 256 & 0.466 & 0.458  \\ 
Siamese-\textit{Adjacent}-\tiny{\textit{InfoNCE-Multi}} & 1280 & 0.450 & 0.446 \\ 
\hline
Siamese-\textit{Random}-\tiny{\textit{InfoNCE}} & 256 & 0.418 & 0.431 \\ 
Siamese-\textit{Random}-\tiny{\textit{InfoNCE-Multi}} & 1280 & 0.436 & 0.461 \\ 
\hline
\textbf{CPC}\tiny{\textit{CPC-InfoNCE}} & 512 & \textbf{0.480} & \textbf{0.491} \\ 
% \hline
% musicnn_{\textit{penultimate}} \cite{musicnn} & 400 & 0.524  & 0.540 \\ 
% \textbf{musicnn}_{\textit{penultimate}} \cite{musicnn} & 400 & \textbf{0.524}  & \textbf{0.540} \\ 
\end{tabular}
\caption{\label{exp-genre} Genre classification results on \textit{FMA small} dataset.
% (\textit{model} - \textit{sampling method} - \textit{loss function}). 
% \textit{TN} denotes the triplet network. 
\textit{Self-aug} denotes the audio augmentation approach, and \textit{Adjacent} denotes positive sampling from the adjacent audio segment. \textit{Random} denotes positive sampling from the entire track.  
\textit{InfoNCE-Multi} denotes \textit{InfoNCE} loss aggregated from multi-level convolutional layer outputs. 
\textit{SVM} denotes a support vector machine classifier with a linear kernel and \textit{LR} denotes a linear logistic regression classifier. \cite{zhang2017split} }

% \end{small}
\end{center}
% \vskip -0.1in
% \vspace{-2mm}
\end{table}

==> tab_inst.tex <==
\begin{table}[t!]
% \vskip 0.15in
\begin{center}
% \begin{small}
\begin{tabular}{lcccc}

\textit{Feature} & \textit{dim.} & \textit{SVM} & \textit{LR} \\ 
\hline
\hline
MFCC & 40 & 0.473 & 0.481 \\ 
\hline
% Siamese-{\textit{track}}_{\textit{Triplet Margin}} & 128 & 0.254 & 0.379 \\ 
% Siamese-{\textit{adjacent}}_{\textit{Triplet Margin}} & 128 & 0.167 & 0.357 \\ 
% \hline
Siamese-{\textit{Self-aug}}-\tiny{\textit{InfoNCE}} & 128 & 0.431 & 0.438  \\ 
Siamese-{\textit{Self-aug}}-\tiny{\textit{InfoNCE-Multi}} & 640 & 0.520 & 0.532 \\ 
\hline
Siamese-{\textit{Adjacent}}-\tiny{\textit{InfoNCE}} & 128 & 0.388 & 0.379 \\
\textbf{Siamese}-{\textbf{\textit{Adjacent}}}-\tiny{\textit{InfoNCE-Multi}} & 640 & \textbf{0.592} & \textbf{0.575} \\
\hline
Siamese-{\textit{Random}}-\tiny{\textit{InfoNCE}} & 128 & 0.374 & 0.361 \\ 
\textbf{Siamese}-{\textbf{\textit{Random}}}-\tiny{\textit{InfoNCE-Multi}} & 640 & \textbf{0.581} & \textbf{0.560} \\
\hline
CPC\tiny{\textit{CPC-InfoNCE}} & 256 & 0.490 & 0.486 \\ 
% \hline
% musicnn_{\textit{penultimate}} \cite{musicnn} & 200 & 0.662 &  0.657 \\ 
% \textbf{musicnn}_{\textit{penultimate}} \cite{musicnn} & 200 & \textbf{0.662} &  \textbf{0.657} \\ 
\end{tabular}
\caption{\label{exp-inst} Instrument classification results on \textit{IRMAS} dataset.
% (\textit{model} - \textit{sampling method} - \textit{loss function}).
% (Abbreviations of model names and classification methods are the same as Table \ref{exp-genre}.)
For all self-supervised embeddings, we do not use mean and standard deviation values since 3 second input is embedded into a single vector.
} 
% \end{small}
\end{center}
% \vskip -0.1in
% \vspace{-3mm}
\end{table}

==> tab_music.tex <==
\begin{table}[t!]
% \vskip 0.15in
\begin{center}
% \begin{small}
\begin{tabular}{lccc}
\textit{Feature} & \textit{dim.} & \textit{HR@10} & \textit{MPR} \\ 
\hline
\hline
MFCC & 40 & 0.196 & 0.381 \\ 
\hline
% Siamese-{\textit{track-}}_{\textit{Triplet Margin}} & 256 & 0.2573 & 0.3282 \\ 
% Siamese-{\textit{adjacent-}}_{\textit{Triplet Margin}} & 256 & 0.2591 & 0.3215 \\ 
% \hline
Siamese-{\textit{Self-aug}}-\tiny{\textit{InfoNCE}} & 256 & 0.250 & 0.339  \\ 
Siamese-{\textit{Self-aug}}-\tiny{\textit{InfoNCE-Multi}} & 1280 & 0.242 & 0.350 \\ 
\hline
% \textbf{Siamese}-{\textit{\textbf{adjacent-}}}_{\textit{InfoNCE}} & 256 & \textbf{0.2791} & \textbf{0.3182} \\

Siamese-{\textit{Adjacent}}-\tiny{\textit{InfoNCE}} & 256 & 0.279 & 0.318 \\
Siamese-{\textit{Adjacent}}-\tiny{\textit{InfoNCE-Multi}} & 1280 & 0.262 & 0.332 \\ 
\hline
Siamese-{\textit{Random}}-\tiny{\textit{InfoNCE}} & 256 & 0.239 & 0.377 \\
Siamese-{\textit{Random}}-\tiny{\textit{InfoNCE-Multi}} & 1280 & 0.260 & 0.330 \\
\hline
\textbf{CPC}\tiny{\textit{CPC-InfoNCE}} & 512 & \textbf{0.280} & \textbf{0.316} \\ 
% \hline
% musicnn_{\textit{penultimate}} \cite{musicnn} & 400 & 0.4460 & 0.2157 \\ 
% \textbf{musicnn}_{\textit{penultimate}} \cite{musicnn} & 200 & \textbf{0.4460} & \textbf{0.2157} \\ 
\end{tabular}
\caption{\label{exp-recomm} Music recommendation results on \textit{AOTM 2011} dataset. 
% (\textit{model} - \textit{sampling method} - \textit{loss function}).
% (Abbreviations of model names are the same as Table \ref{exp-genre}.) 
\textit{HR@10} denotes Hit ratio at 10 (higher the better), and \textit{MPR} denotes mean percentile rank (lower the better).
Results are averaged over 10 runs.
} 
% \end{small}
\end{center}
% \vskip -0.1in
% \vspace{-4mm}
\end{table}
